Evaluating Reinforcement Learning Safety and Trustworthiness in Cyber-Physical Systems

Cyber-Physical Systems (CPS) often leverage Reinforcement Learning (RL) techniques to adapt dynamically to changing environments and optimize performance. However, it is challenging to construct safety cases for RL components. We therefore propose the SAFE-RL (Safety and Accountability Framework for Evaluating Reinforcement Learning) for supporting the development, validation, and safe deployment of RL-based CPS. We adopt a design science approach to construct the framework and demonstrate its use in three RL applications in small Uncrewed Aerial systems (sUAS)

==> 4_related-work.tex <==
\section{Related-Work}
\label{sec:related}
%Existing frameworks include SARL \cite{MiretSARL} and MOSAIC \cite{BacciProbGaurantee} which incorporate safety via reinforcement or probabilistic guarantees in specific environments. In contrast, our approach offers a systematic process for stakeholders to assess risks, establish guidelines, and validate safety comprehensively. 
While several existing standards focus on AI safety, they do not specifically address the challenges of RL. Similarly, checklist-based frameworks, such as the AI Safety and Security Checklist by HackerOne \cite{checklist1} and the LivePerson AI System Safety Checklist \cite{checklist2}, offer a structured approach to safety analysis but are also not tailored to RL systems. %Finally, Safety Assurance Cases \cite{fraunhofer2021safeai},  l for measurable AI safety outcomes. In contrast, to prior work on trustworthy ML \framework provides a structured process for evaluating RL system safety, articulating design decisions, and systematically validating trustworthiness.

==> 5_threats.tex <==
\section{Threats to Validity}
\label{sec:threats}
Internal validity refers to the rigor of the experimental design and the extent to which results are due to interventions rather than confounding factors. A limitation of our study is the inclusion of only three experts, potentially resulting in insufficient diversity of perspectives. Additionally, there is a risk of confirmation bias in their feedback. To mitigate this, we structured questions to encourage critical evaluation, explicitly inviting the experts to identify areas for improvement and to highlight both strengths and weaknesses of the framework.

External validity concerns the generalizability of our findings. Although our framework was designed to be relevant across various types of CPS, it has so far been applied only to small autonomous vehicles (both ground and aerial). Notably, the sUAS case studies involve real-world systems prioritizing challenges such as maintaining minimum separation distances and optimizing economical routes. Future work will extend the application of \framework to additional types of CPS and, building on positive feedback, explore frameworks tailored to different AI algorithmic domains.

Construct validity reflects how well the study measures the intended variables and concepts. By adopting Design Science, we integrated evaluation into an iterative process, evolving the framework based on intermediate findings. However, the final evaluation, due to the time-intensive nature of applying the framework (approximately one hour per use case), relied on expert inspection of a pre-existing use case and included only three experts. Moving forward, we will incorporate the suggested improvements and invite broader participation to test \framework in diverse scenarios.

==> figures/exampe-branch.tex <==
\begin{figure}
    \centering
   
    \includegraphics[width=\columnwidth]{figures/images/resilience-and-adaptation.png}
     \caption{The \framework framework structures the analysis into a hierarchy of goals, subgoals, questions (\texttt{ASK}), and evidence nodes. The complete framework is provided in the appendix.}    
    \label{fig:example-branch}
    \vspace{-8pt}
\end{figure}

==> figures/goals-zoomed-in.tex <==
% Define the custom color
\definecolor{teal}{HTML}{9AB8C2}
\definecolor{green1}{HTML}{9CBCA3}
\definecolor{rosepink}{HTML}{d398cb}
\begin{figure*}[h]
    \centering
    % Three Stacked Subfigures in Color Boxes
    \begin{subfigure}{0.85\textwidth}
        \begin{tcolorbox}[colback=teal!20!white, colframe=teal!80!black, width=\textwidth, boxrule=0.3mm, left=1mm, right=1mm, top=1mm, bottom=1mm]
            \includegraphics[width=\textwidth]{figures/images/goal1.png} % Replace with your image path
        \end{tcolorbox}
        \caption{Goal 1}
    \end{subfigure}

    \begin{subfigure}{0.85\textwidth}
        \begin{tcolorbox}[colback=green1!10!white, colframe=green1!80!black, width=\textwidth, boxrule=0.5mm, left=1mm, right=1mm, top=1mm, bottom=1mm]
            \includegraphics[width=\textwidth]{figures/images/goal2.png} % Replace with your image path
        \end{tcolorbox}
        \caption{Goal 2}
    \end{subfigure}

    \begin{subfigure}{0.67\textwidth}
        \begin{tcolorbox}[colback=rosepink!10!white, colframe=rosepink!80!black, width=\textwidth, boxrule=0.5mm, left=1mm, right=1mm, top=1mm, bottom=1mm]
            \includegraphics[width=\textwidth]{figures/images/goal3.png} % Replace with your image path
        \end{tcolorbox}
        \caption{Goal 3}
    \end{subfigure}

    \caption{Subtrees of subgoals, \texttt{ASKS}, and evidence for the three top-level goals in the \framework framework.}
    \label{fig:goals-zoomed}
\end{figure*}

==> figures/gv/decision-tree-v2.tex <==
digraph SafetyArguments {
    node [shape=rect, style=filled, fontname="Helvetica", fontsize=16, fillcolor="#FAD7A0"];
    edge [fontname="Helvetica", fontsize=14];
    ranksep=.2
    nodesep=.1

    // GOALS and SUBGOALS First
    N1 [label="CONTEXT:\n Reinforcement Learning has been used to train\n the actions of a single or multi-agent CPS \noperating in a safety-critical domain.", style="dashed"]

    N2[label=<
    <TABLE BORDER="0" CELLBORDER="1" CELLSPACING="0" CELLPADDING="4" BGCOLOR="white">
    <TR><TD ALIGN="CENTER" BGCOLOR="#E6F2FA" BORDER="1" COLOR="#A3B7C5"><b>GOAL 1: <BR/>Environment Alignment</b></TD></TR>
    <TR><TD ALIGN="CENTER" BGCOLOR="#E6F2FA" BORDER="1" COLOR="#A3B7C5">Model is selected for <BR/> and trained in a <BR/>realistic environment</TD></TR>
    </TABLE>
    >, fillcolor="white", color="white"]; 
    
     N3[label=<
    <TABLE BORDER="0" CELLBORDER="1" CELLSPACING="0" CELLPADDING="4" BGCOLOR="white">
    <TR><TD ALIGN="CENTER" BGCOLOR="#E6F2FA" BORDER="1" COLOR="#A3B7C5"><b>Subgoal 1.1: <BR/>Scenario Variety</b></TD></TR>
    <TR><TD ALIGN="CENTER" BGCOLOR="#E6F2FA" BORDER="1" COLOR="#A3B7C5">Training covers <BR/>real-world scenarios <BR/>including edge cases</TD></TR>
    </TABLE>
    >, fillcolor="white", color="white"];
    
    //The RL agent’s decision-making process is transparent for human-on-the-loop supervisors
    
    
    N48[label=<
    <TABLE BORDER="1" CELLBORDER="1" CELLSPACING="0" CELLPADDING="4" BGCOLOR="#D7E6D3">
    <TR><TD ALIGN="CENTER" BGCOLOR="#D7E6D3"><b>ASK (15)</b></TD></TR>
    <TR><TD ALIGN="CENTER">If possible, is the <BR/>human overseer actively<BR/> involved in shaping  <BR/> the training process to  <BR/> enhance transparency &amp; <BR/> promote alignment with <BR/>specific safety &amp;<BR/> operational goals?<BR/></TD></TR>
    <TR><TD ALIGN="CENTER">☐ Yes | ☐ No | ☐ ? | ☐ N/A</TD></TR></TABLE>
    >, fillcolor="white", color="white"];
 
    N28[label=<
    <TABLE BORDER="0" CELLBORDER="1" CELLSPACING="0" CELLPADDING="4" BGCOLOR="white">
    <TR><TD ALIGN="CENTER" BGCOLOR="#E6F2FA" BORDER="1" COLOR="#A3B7C5"><b>Subgoal 3.2: <BR/>Transparency</b></TD></TR>
    <TR><TD ALIGN="CENTER" BGCOLOR="#E6F2FA" BORDER="1" COLOR="#A3B7C5">Human overseer has insight<BR/>into policy and value functions <BR/>&amp; safety compliance</TD></TR>
    </TABLE>
    >, fillcolor="white", color="white"];

    N31[label=<
    <TABLE BORDER="1" CELLBORDER="1" CELLSPACING="0" CELLPADDING="4" BGCOLOR="#D7E6D3">
    <TR><TD ALIGN="CENTER" BGCOLOR="#D7E6D3"><b>ASK (16)</b></TD></TR>
    <TR><TD ALIGN="CENTER">Are critical factors or<BR/>states that significantly <BR/>impact behavior and safety <BR/> highlighted for the <BR/>human overseer?<BR/></TD></TR>
    <TR><TD ALIGN="CENTER">☐ Yes | ☐ No | ☐ ? | ☐ N/A</TD></TR></TABLE>
    >, fillcolor="white", color="white"];
    
        N46[label=<
    <TABLE BORDER="1" CELLBORDER="1" CELLSPACING="0" CELLPADDING="4" BGCOLOR="#D7E6D3">
    <TR><TD ALIGN="CENTER" BGCOLOR="#D7E6D3"><b>ASK (17)</b></TD></TR>
    <TR><TD ALIGN="CENTER">Are reward, value,  <BR/>and/or policy functions,<BR/>along with safety criteria, <BR/>exposed to the <BR/> human overseer<BR/>during runtime to ensure <BR/> safety compliance?<BR/></TD></TR>
    <TR><TD ALIGN="CENTER">☐ Yes | ☐ No | ☐ ? | ☐ N/A</TD></TR></TABLE>
    >, fillcolor="white", color="white"];

    N34 [label=<
        <TABLE BORDER="0" CELLBORDER="1" CELLSPACING="0" CELLPADDING="4" BGCOLOR="#FAD7A0">
            <TR><TD WIDTH="20" ALIGN="CENTER" BGCOLOR="#FAD7A0" BORDER="0" COLOR="#A5B39E">☐</TD><TD WIDTH="100" ALIGN="LEFT" BGCOLOR="#FAD7A0" BORDER="0" COLOR="#A5B39E">Hazard analysis</TD></TR>
            <TR><TD WIDTH="20" ALIGN="CENTER" BGCOLOR="#FAD7A0" BORDER="0" COLOR="#A5B39E">☐</TD><TD WIDTH="100" ALIGN="LEFT" BGCOLOR="#FAD7A0" BORDER="0" COLOR="#A5B39E">Design &amp; rationale</TD></TR>
            <TR><TD WIDTH="20" ALIGN="CENTER" BGCOLOR="#FAD7A0" BORDER="0" COLOR="#A5B39E">☐</TD><TD WIDTH="100" ALIGN="LEFT" BGCOLOR="#FAD7A0" BORDER="0" COLOR="#A5B39E">User study outcomes</TD></TR>
        </TABLE>
    >,fillcolor="#FAD7A0"];
    
        N19[label=<
    <TABLE BORDER="1" CELLBORDER="1" CELLSPACING="0" CELLPADDING="4" BGCOLOR="#D7E6D3">
    <TR><TD ALIGN="CENTER" BGCOLOR="#E6F2FA" BORDER="1" COLOR="#A3B7C5"><b>GOAL 2<BR/>Safety</b></TD></TR>
    <TR><TD ALIGN="CENTER" BGCOLOR="#E6F2FA" BORDER="1" COLOR="#A3B7C5">Safety prioritization <BR/>during RL training<BR/> and deployment</TD></TR></TABLE>
    >, fillcolor="white", color="white"];    
    
        N25[label=<
    <TABLE BORDER="1" CELLBORDER="1" CELLSPACING="0" CELLPADDING="4" BGCOLOR="#D7E6D3">
    <TR><TD ALIGN="CENTER" BGCOLOR="#E6F2FA" BORDER="1" COLOR="#A3B7C5"><b>Subgoal 2.2 </b></TD></TR>
    <TR><TD ALIGN="CENTER" BGCOLOR="#E6F2FA" BORDER="1" COLOR="#A3B7C5">Incorporate safety<BR/> considerations in<BR/>RL training</TD></TR></TABLE>
    >, fillcolor="white", color="white"]; 
    
    
    N36[label=<
    <TABLE BORDER="1" CELLBORDER="1" CELLSPACING="0" CELLPADDING="4" BGCOLOR="#D7E6D3">
    <TR><TD ALIGN="CENTER" BGCOLOR="#D7E6D3"><b>ASK (12) </b></TD></TR>
    <TR><TD ALIGN="CENTER">Does the reward function<BR/>incorporate penalties<BR/>for un-safe actions?</TD></TR>
    <TR><TD ALIGN="CENTER">☐ Yes | ☐ No | ☐ ? | ☐ N/A</TD></TR></TABLE>
    >, fillcolor="white", color="white"];  
    
    
    N42[label=<
    <TABLE BORDER="1" CELLBORDER="1" CELLSPACING="0" CELLPADDING="4" BGCOLOR="#D7E6D3">
    <TR><TD ALIGN="CENTER" BGCOLOR="#D7E6D3"><b>ASK (13) </b></TD></TR>
    <TR><TD ALIGN="CENTER">Are safety constraints <BR/>integrated into the policy<BR/> optimization/training<BR/> process to align with <BR/>safety requirements?</TD></TR>
    <TR><TD ALIGN="CENTER">☐ Yes | ☐ No | ☐ ? | ☐ N/A</TD></TR></TABLE>
    >, fillcolor="white", color="white"];  
    
        N49[label=<
    <TABLE BORDER="1" CELLBORDER="1" CELLSPACING="0" CELLPADDING="4" BGCOLOR="#D7E6D3">
    <TR><TD ALIGN="CENTER" BGCOLOR="#D7E6D3"><b>ASK (11) </b></TD></TR>
    <TR><TD ALIGN="CENTER">Do the training and <BR/>evaluation metrics explicitly<BR/> include measures of safety?<BR/></TD></TR>
    <TR><TD ALIGN="CENTER">☐ Yes | ☐ No | ☐ ? | ☐ N/A</TD></TR></TABLE>
    >, fillcolor="white", color="white"];
    
    N12[label=<
    <TABLE BORDER="1" CELLBORDER="1" CELLSPACING="0" CELLPADDING="4" BGCOLOR="#D7E6D3">
    <TR><TD ALIGN="CENTER" BGCOLOR="#E6F2FA" BORDER="1" COLOR="#A3B7C5"><b>Subgoal 2.1 </b></TD></TR>
    <TR><TD ALIGN="CENTER" BGCOLOR="#E6F2FA" BORDER="1" COLOR="#A3B7C5">Establish a safety<BR/>envelope during<BR/>runtime to overcome<BR/>potential training <BR/>shortcomings.</TD></TR></TABLE>
    >, fillcolor="white", color="white"];     
    
    
    N29[label=<
    <TABLE BORDER="0" CELLBORDER="1" CELLSPACING="0" CELLPADDING="4" BGCOLOR="white">
    <TR><TD ALIGN="CENTER" BGCOLOR="#E6F2FA" BORDER="1" COLOR="#A3B7C5"><b>Subgoal 3.1: <BR/>Human Intervention</b></TD></TR>
    <TR><TD ALIGN="CENTER" BGCOLOR="#E6F2FA" BORDER="1" COLOR="#A3B7C5">Human overseer has <BR/>affordances to safely<BR/>intervene when needed</TD></TR>
    </TABLE>
    >, fillcolor="white", color="white"];
    
    N32[label=<
    <TABLE BORDER="1" CELLBORDER="1" CELLSPACING="0" CELLPADDING="4" BGCOLOR="#D7E6D3">
    <TR><TD ALIGN="CENTER" BGCOLOR="#D7E6D3"><b>ASK (18)</b></TD></TR>
    <TR><TD ALIGN="CENTER">Have human interventions<BR/>been identified &amp; supported <BR/>by affordances?</TD></TR>
    <TR><TD ALIGN="CENTER">☐ Yes | ☐ No | ☐ ? | ☐ N/A</TD></TR></TABLE>
    >, fillcolor="white", color="white"];    
    
    N30[label=<
    <TABLE BORDER="0" CELLBORDER="1" CELLSPACING="0" CELLPADDING="4" BGCOLOR="white">
    <TR><TD ALIGN="CENTER" BGCOLOR="#E6F2FA" BORDER="1" COLOR="#A3B7C5"><b>Subgoal 3.3: <BR/>Post-mortem inspection</b></TD></TR>
    <TR><TD ALIGN="CENTER" BGCOLOR="#E6F2FA" BORDER="1" COLOR="#A3B7C5">The system supports<BR/>post-mortem analysis<BR/>of RL-driven behavior</TD></TR>
    </TABLE>
    >, fillcolor="white", color="white"];
    
    N33[label=<
    <TABLE BORDER="1" CELLBORDER="1" CELLSPACING="0" CELLPADDING="4" BGCOLOR="#D7E6D3">
    <TR><TD ALIGN="CENTER" BGCOLOR="#D7E6D3"><b>ASK (14)</b></TD></TR>
    <TR><TD ALIGN="CENTER">Are clear and detailed<BR/>logs, metrics, and<BR/>indicators available to<BR/>trace decision-making <BR/> and faciliate analysis of <BR/>issues post-mortem?</TD></TR>
    <TR><TD ALIGN="CENTER">☐ Yes | ☐ No | ☐ ? | ☐ N/A</TD></TR></TABLE>
    >, fillcolor="white", color="white"]; 
    
    N35 [label=<
        <TABLE BORDER="0" CELLBORDER="1" CELLSPACING="0" CELLPADDING="4" BGCOLOR="#FAD7A0">
            <TR><TD WIDTH="20" ALIGN="CENTER" BGCOLOR="#FAD7A0" BORDER="0" COLOR="#A5B39E">☐</TD><TD WIDTH="100" ALIGN="LEFT" BGCOLOR="#FAD7A0" BORDER="0" COLOR="#A5B39E">Design &amp; rationale</TD></TR>
            <TR><TD WIDTH="20" ALIGN="CENTER" BGCOLOR="#FAD7A0" BORDER="0" COLOR="#A5B39E">☐</TD><TD WIDTH="100" ALIGN="LEFT" BGCOLOR="#FAD7A0" BORDER="0" COLOR="#A5B39E">User study outcomes</TD></TR>
        </TABLE>
    >,fillcolor="#FAD7A0"];


    N4[label=<
    <TABLE BORDER="0" CELLBORDER="1" CELLSPACING="0" CELLPADDING="4" BGCOLOR="white">
    <TR><TD ALIGN="CENTER" BGCOLOR="#E6F2FA" BORDER="1" COLOR="#A3B7C5"><b>Subgoal 1.2: <BR/>Novel Scenarios</b></TD></TR>
    <TR><TD ALIGN="CENTER" BGCOLOR="#E6F2FA" BORDER="1" COLOR="#A3B7C5">The system will detect &amp;<BR/>handle novel scenarios <BR/>at runtime.</TD></TR>
    </TABLE>
    >, fillcolor="white", color="white"];
    
    N27[label=<
    <TABLE BORDER="0" CELLBORDER="1" CELLSPACING="0" CELLPADDING="4" BGCOLOR="white">
    <TR><TD ALIGN="CENTER" BGCOLOR="#E6F2FA" BORDER="1" COLOR="#A3B7C5"><b>GOAL 3: <BR/>Transparent &amp; Explainable</b></TD></TR>
    <TR><TD ALIGN="CENTER" BGCOLOR="#E6F2FA" BORDER="1" COLOR="#A3B7C5">Expose information<BR/>needed by users to <BR/>promote trust &amp; oversight<BR/>in the RL trained model</TD></TR>
    </TABLE>
    >, fillcolor="white", color="white"];
    

    

 //The system is explainable and transparent, ensuring trust and oversight
    // ASK Second
    N7[label=<
    <TABLE BORDER="1" CELLBORDER="1" CELLSPACING="0" CELLPADDING="4" BGCOLOR="#D7E6D3">
    <TR><TD ALIGN="CENTER" BGCOLOR="#D7E6D3"><b>ASK (1) </b></TD></TR>
    <TR><TD ALIGN="CENTER">Have the risks associated<br/>with mismatched training<br/>scenarios been identified<br/>and addressed?</TD></TR>
    <TR><TD ALIGN="CENTER">☐ Yes | ☐ No | ☐ ? | ☐ N/A</TD></TR></TABLE>
    >, fillcolor="white", color="white"];
    
    N26[label=<
    <TABLE BORDER="1" CELLBORDER="1" CELLSPACING="0" CELLPADDING="4" BGCOLOR="#D7E6D3">
    <TR><TD ALIGN="CENTER" BGCOLOR="#D7E6D3"><b>ASK (9)</b></TD></TR>
    <TR><TD ALIGN="CENTER">Is the architecture <BR/>designed with <BR/>fault tolerance mechanisms<BR/> and failsafes to manage <BR/> unforseen RL failures?</TD></TR>
    <TR><TD ALIGN="CENTER">☐ Yes | ☐ No | ☐ ? | ☐ N/A</TD></TR></TABLE>
    >, fillcolor="white", color="white"];
    
            N9[label=<
    <TABLE BORDER="1" CELLBORDER="1" CELLSPACING="0" CELLPADDING="4" BGCOLOR="#D7E6D3">
    <TR><TD ALIGN="CENTER" BGCOLOR="#D7E6D3"><b>ASK (5)</b></TD></TR>
    <TR><TD ALIGN="CENTER">Is there sufficient evidence<br/>that RL training scenerios<br/>comprehensively cover all <br/>identified scenarios?</TD></TR>
    <TR><TD ALIGN="CENTER">☐ Yes | ☐ No | ☐ ? | ☐ N/A</TD></TR></TABLE>
    >, fillcolor="white", color="white"];
    
        
    N38[label=<
    <TABLE BORDER="1" CELLBORDER="1" CELLSPACING="0" CELLPADDING="4" BGCOLOR="#D7E6D3">
    <TR><TD ALIGN="CENTER" BGCOLOR="#D7E6D3"><b>ASK (0) </b></TD></TR>
    <TR><TD ALIGN="CENTER">Does the proposed RL agent<br/>align with the environment&apos;s<br/>characteristics, such as<br/>observability, continuity,<br/>and state representation?</TD></TR>
    <TR><TD ALIGN="CENTER">☐ Yes | ☐ No | ☐ ? | ☐ N/A</TD></TR></TABLE>
    >, fillcolor="white", color="white"];

    N8[label=<
    <TABLE BORDER="1" CELLBORDER="1" CELLSPACING="0" CELLPADDING="4" BGCOLOR="#D7E6D3">
    <TR><TD ALIGN="CENTER" BGCOLOR="#D7E6D3"><b>ASK (2)</b></TD></TR>
    <TR><TD ALIGN="CENTER">Is there sufficient evidence<br/>that normal, abnormal &amp;<br/>possible edge scenarios<br/> have been identified, <br/>including variations in  <br/>sensor inputs, <br/>system states, or<br/> environmental factors?</TD></TR>
    <TR><TD ALIGN="CENTER">☐ Yes | ☐ No | ☐ ? | ☐ N/A</TD></TR></TABLE>
    >, fillcolor="white", color="white"];
    
            N40[label=<
    <TABLE BORDER="1" CELLBORDER="1" CELLSPACING="0" CELLPADDING="4" BGCOLOR="#D7E6D3">
    <TR><TD ALIGN="CENTER" BGCOLOR="#D7E6D3"><b>ASK (3)</b></TD></TR>
    <TR><TD ALIGN="CENTER">Have the differences<br/>between similuated &amp; <br/>real world environments<br/> been identified and <br/>addressed?</TD></TR>
    <TR><TD ALIGN="CENTER">☐ Yes | ☐ No | ☐ ? | ☐ N/A</TD></TR></TABLE>
    >, fillcolor="white", color="white"];
    
    
    N44[label=<
    <TABLE BORDER="1" CELLBORDER="1" CELLSPACING="0" CELLPADDING="4" BGCOLOR="#D7E6D3">
    <TR><TD ALIGN="CENTER" BGCOLOR="#D7E6D3"><b>ASK (4)</b></TD></TR>
    <TR><TD ALIGN="CENTER">In multi-agent training,<br/>are individual RL-agents<br/>equipped to detect &amp; adapt to<br/>failures of other agents?</TD></TR>
    <TR><TD ALIGN="CENTER">☐ Yes | ☐ No | ☐ ? | ☐ N/A</TD></TR></TABLE>
    >, fillcolor="white", color="white"];

        

    
    

//The reward function is explicitly designed to prioritize safety    
//     Claim 4.2: Redundancy mechanisms mitigate risk where formal guarantees are not feasible.
// Sub-claim 4.2.1: Redundancy mechanisms, such as secondary control systems or human oversight, are in place for safety-critical actions.
// Sub-claim 4.2.2: Backup systems have been tested to ensure they perform reliably when the RL agent encounters unsafe scenarios.
    
    N22[label=<
    <TABLE BORDER="1" CELLBORDER="1" CELLSPACING="0" CELLPADDING="4" BGCOLOR="#D7E6D3">
    <TR><TD ALIGN="CENTER" BGCOLOR="#D7E6D3"><b>ASK (10) </b></TD></TR>
    <TR><TD ALIGN="CENTER">Have safety constraints <BR/>been established that,<BR/>if upheld, would prevent<BR/> all predictable unsafe<BR/> behavior at runtime?</TD></TR>
    <TR><TD ALIGN="CENTER">☐ Yes | ☐ No | ☐ ? | ☐ N/A</TD></TR></TABLE>
    >, fillcolor="white", color="white"];    

    
    N20[label=<
    <TABLE BORDER="0" CELLBORDER="1" CELLSPACING="0" CELLPADDING="4" BGCOLOR="white">
    <TR><TD ALIGN="CENTER" BGCOLOR="#E6F2FA" BORDER="1" COLOR="#A3B7C5"><b>TOP LEVEL GOAL</b></TD></TR>
    <TR><TD ALIGN="CENTER" BGCOLOR="#E6F2FA" BORDER="1" COLOR="#A3B7C5">Correct &amp; Safe behavior of <BR/>RL trained system</TD></TR>
    </TABLE>
    >, fillcolor="white", color="white"]; 


    N11[label=<
    <TABLE BORDER="1" CELLBORDER="1" CELLSPACING="0" CELLPADDING="4" BGCOLOR="#D7E6D3">
    <TR><TD ALIGN="CENTER" BGCOLOR="#D7E6D3"><b>ASK (8)</b></TD></TR>
    <TR><TD ALIGN="CENTER">Can the system detect,<br/>diagnose, and mitigate<br/>unwanted behavior, <BR/>including constraint violations <BR/>deviations from expected policy, <BR/> &amp; other unexpected actions?</TD></TR>
    <TR><TD ALIGN="CENTER">☐ Yes | ☐ No | ☐ ? | ☐ N/A</TD></TR></TABLE>
    >, fillcolor="white", color="white"];
    
    // N21[label=<
    // <TABLE BORDER="1" CELLBORDER="1" CELLSPACING="0" CELLPADDING="4" BGCOLOR="#D7E6D3">
    // <TR><TD ALIGN="CENTER" BGCOLOR="#D7E6D3"><b>ASK</b></TD></TR>
    // <TR><TD ALIGN="CENTER">Can the system detect,<br/>constraint violations?</TD></TR>
    // <TR><TD ALIGN="CENTER">☐ Yes | ☐ No | ☐ ? | ☐ N/A</TD></TR></TABLE>
    // >, fillcolor="white", color="white"];

    N6[label=<
    <TABLE BORDER="1" CELLBORDER="1" CELLSPACING="0" CELLPADDING="4" BGCOLOR="#D7E6D3">
    <TR><TD ALIGN="CENTER" BGCOLOR="#D7E6D3"><b>ASK (6)</b></TD></TR>
    <TR><TD ALIGN="CENTER">Is there sufficient evidence<br/>that the system is designed<br/>to detect if untrained<br/> or adversarial scenerios<br/> are encountered?</TD></TR>
    <TR><TD ALIGN="CENTER">☐ Yes | ☐ No | ☐ ? | ☐ N/A</TD></TR></TABLE>
    >, fillcolor="white", color="white"];

    N13 [label=<
        <TABLE BORDER="0" CELLBORDER="1" CELLSPACING="0" CELLPADDING="4" BGCOLOR="#D7E6D3">
            <TR><TD ALIGN="CENTER" BGCOLOR="#D7E6D3" BORDER="1" COLOR="#A3B7C5"><b>ASK (7)</b></TD></TR>
            <TR><TD ALIGN="CENTER" BGCOLOR="#D7E6D3" BORDER="1" COLOR="#A3B7C5">Have appropriate failsafes<BR/>been established to address<BR/>system failures due to<BR/>unexpected scenarios?</TD></TR>
            <TR><TD ALIGN="CENTER">☐ Yes | ☐ No | ☐ ? | ☐ N/A</TD></TR>
        </TABLE>
    >, fillcolor="white", color="white"];

// EVIDENCE Last
N14 [label=<
    <TABLE BORDER="0" CELLBORDER="1" CELLSPACING="0" CELLPADDING="4" BGCOLOR="#FAD7A0">
        <TR><TD WIDTH="20" ALIGN="CENTER" BGCOLOR="#FAD7A0" BORDER="0" COLOR="#A5B39E">☐</TD><TD WIDTH="100" ALIGN="LEFT" BGCOLOR="#FAD7A0" BORDER="0" COLOR="#A5B39E">Hazard Analysis</TD></TR>
        <TR><TD WIDTH="20" ALIGN="CENTER" BGCOLOR="#FAD7A0" BORDER="0" COLOR="#A5B39E">☐</TD><TD WIDTH="100" ALIGN="LEFT" BGCOLOR="#FAD7A0" BORDER="0" COLOR="#A5B39E">List (mtg notes)</TD></TR>
        <TR><TD WIDTH="20" ALIGN="CENTER" BGCOLOR="#FAD7A0" BORDER="0" COLOR="#A5B39E">☐</TD><TD WIDTH="100" ALIGN="LEFT" BGCOLOR="#FAD7A0" BORDER="0" COLOR="#A5B39E">Use Case docs</TD></TR>
    </TABLE>
>,fillcolor="#FAD7A0"];

N15 [label=<
    <TABLE BORDER="0" CELLBORDER="1" CELLSPACING="0" CELLPADDING="4" BGCOLOR="#FAD7A0">
        <TR><TD WIDTH="20" ALIGN="CENTER" BGCOLOR="#FAD7A0" BORDER="0" COLOR="#A5B39E">☐</TD><TD WIDTH="100" ALIGN="LEFT" BGCOLOR="#FAD7A0" BORDER="0" COLOR="#A5B39E">Scen. Coverage Matrix</TD></TR>
        <TR><TD WIDTH="20" ALIGN="CENTER" BGCOLOR="#FAD7A0" BORDER="0" COLOR="#A5B39E">☐</TD><TD WIDTH="100" ALIGN="LEFT" BGCOLOR="#FAD7A0" BORDER="0" COLOR="#A5B39E">Sim. Training logs</TD></TR>
    </TABLE>
>,fillcolor="#FAD7A0"];

N16 [label=<
    <TABLE BORDER="0" CELLBORDER="1" CELLSPACING="0" CELLPADDING="4" BGCOLOR="#FAD7A0">
        <TR><TD WIDTH="20" ALIGN="CENTER" BGCOLOR="#FAD7A0" BORDER="0" COLOR="#A5B39E">☐</TD><TD WIDTH="100" ALIGN="LEFT" BGCOLOR="#FAD7A0" BORDER="0" COLOR="#A5B39E">Design Rationale</TD></TR>
        <TR><TD WIDTH="20" ALIGN="CENTER" BGCOLOR="#FAD7A0" BORDER="0" COLOR="#A5B39E">☐</TD><TD WIDTH="100" ALIGN="LEFT" BGCOLOR="#FAD7A0" BORDER="0" COLOR="#A5B39E">Runtime Monitor List</TD></TR>
    </TABLE>
>,fillcolor="#FAD7A0"];

N17 [label=<
    <TABLE BORDER="0" CELLBORDER="1" CELLSPACING="0" CELLPADDING="4" BGCOLOR="#FAD7A0">
        <TR><TD WIDTH="20" ALIGN="CENTER" BGCOLOR="#FAD7A0" BORDER="0" COLOR="#A5B39E">☐</TD><TD WIDTH="100" ALIGN="LEFT" BGCOLOR="#FAD7A0" BORDER="0" COLOR="#A5B39E">Simulation design</TD></TR>
        <TR><TD WIDTH="20" ALIGN="CENTER" BGCOLOR="#FAD7A0" BORDER="0" COLOR="#A5B39E">☐</TD><TD WIDTH="100" ALIGN="LEFT" BGCOLOR="#FAD7A0" BORDER="0" COLOR="#A5B39E">Test results</TD></TR>
        <TR><TD WIDTH="20" ALIGN="CENTER" BGCOLOR="#FAD7A0" BORDER="0" COLOR="#A5B39E">☐</TD><TD WIDTH="100" ALIGN="LEFT" BGCOLOR="#FAD7A0" BORDER="0" COLOR="#A5B39E">Field logs</TD></TR>
    </TABLE>
>,fillcolor="#FAD7A0"];

N18 [label=<
    <TABLE BORDER="0" CELLBORDER="1" CELLSPACING="0" CELLPADDING="4" BGCOLOR="#FAD7A0">
        <TR><TD WIDTH="20" ALIGN="CENTER" BGCOLOR="#FAD7A0" BORDER="0" COLOR="#A5B39E">☐</TD><TD WIDTH="100" ALIGN="LEFT" BGCOLOR="#FAD7A0" BORDER="0" COLOR="#A5B39E">List anomaly monitors</TD></TR>
        <TR><TD WIDTH="20" ALIGN="CENTER" BGCOLOR="#FAD7A0" BORDER="0" COLOR="#A5B39E">☐</TD><TD WIDTH="100" ALIGN="LEFT" BGCOLOR="#FAD7A0" BORDER="0" COLOR="#A5B39E">Tests &amp; outcomes</TD></TR>
        <TR><TD WIDTH="20" ALIGN="CENTER" BGCOLOR="#FAD7A0" BORDER="0" COLOR="#A5B39E">☐</TD><TD WIDTH="100" ALIGN="LEFT" BGCOLOR="#FAD7A0" BORDER="0" COLOR="#A5B39E">Field logs</TD></TR>
    </TABLE>
>,fillcolor="#FAD7A0"];

N23 [label=<
    <TABLE BORDER="0" CELLBORDER="1" CELLSPACING="0" CELLPADDING="4" BGCOLOR="#FAD7A0">
        <TR><TD WIDTH="20" ALIGN="CENTER" BGCOLOR="#FAD7A0" BORDER="0" COLOR="#A5B39E">☐</TD><TD WIDTH="100" ALIGN="LEFT" BGCOLOR="#FAD7A0" BORDER="0" COLOR="#A5B39E">Architectural risks</TD></TR>
        <TR><TD WIDTH="20" ALIGN="CENTER" BGCOLOR="#FAD7A0" BORDER="0" COLOR="#A5B39E">☐</TD><TD WIDTH="100" ALIGN="LEFT" BGCOLOR="#FAD7A0" BORDER="0" COLOR="#A5B39E">ATAM</TD></TR>
        <TR><TD WIDTH="20" ALIGN="CENTER" BGCOLOR="#FAD7A0" BORDER="0" COLOR="#A5B39E">☐</TD><TD WIDTH="100" ALIGN="LEFT" BGCOLOR="#FAD7A0" BORDER="0" COLOR="#A5B39E">Design docs &amp; rationale</TD></TR>
        <TR><TD WIDTH="20" ALIGN="CENTER" BGCOLOR="#FAD7A0" BORDER="0" COLOR="#A5B39E">☐</TD><TD WIDTH="100" ALIGN="LEFT" BGCOLOR="#FAD7A0" BORDER="0" COLOR="#A5B39E">Test results</TD></TR>
    </TABLE>
>,fillcolor="#FAD7A0"];

N24 [label=<
    <TABLE BORDER="0" CELLBORDER="1" CELLSPACING="0" CELLPADDING="4" BGCOLOR="#FAD7A0">
        <TR><TD WIDTH="20" ALIGN="CENTER" BGCOLOR="#FAD7A0" BORDER="0" COLOR="#A5B39E">☐</TD><TD WIDTH="100" ALIGN="LEFT" BGCOLOR="#FAD7A0" BORDER="0" COLOR="#A5B39E">FMECA</TD></TR>
        <TR><TD WIDTH="20" ALIGN="CENTER" BGCOLOR="#FAD7A0" BORDER="0" COLOR="#A5B39E">☐</TD><TD WIDTH="100" ALIGN="LEFT" BGCOLOR="#FAD7A0" BORDER="0" COLOR="#A5B39E">Constraints list</TD></TR>
    </TABLE>
>,fillcolor="#FAD7A0"];

N37 [label=<
    <TABLE BORDER="0" CELLBORDER="1" CELLSPACING="0" CELLPADDING="4" BGCOLOR="#FAD7A0">
        <TR><TD WIDTH="20" ALIGN="CENTER" BGCOLOR="#FAD7A0" BORDER="0" COLOR="#A5B39E">☐</TD><TD WIDTH="100" ALIGN="LEFT" BGCOLOR="#FAD7A0" BORDER="0" COLOR="#A5B39E">RL specification</TD></TR>
        <TR><TD WIDTH="20" ALIGN="CENTER" BGCOLOR="#FAD7A0" BORDER="0" COLOR="#A5B39E">☐</TD><TD WIDTH="100" ALIGN="LEFT" BGCOLOR="#FAD7A0" BORDER="0" COLOR="#A5B39E">Test results</TD></TR>
                <TR><TD WIDTH="20" ALIGN="CENTER" BGCOLOR="#FAD7A0" BORDER="0" COLOR="#A5B39E">☐</TD><TD WIDTH="100" ALIGN="LEFT" BGCOLOR="#FAD7A0" BORDER="0" COLOR="#A5B39E">Policy Audits</TD></TR>
        <TR><TD WIDTH="20" ALIGN="CENTER" BGCOLOR="#FAD7A0" BORDER="0" COLOR="#A5B39E">☐</TD><TD WIDTH="100" ALIGN="LEFT" BGCOLOR="#FAD7A0" BORDER="0" COLOR="#A5B39E">Training Logs &amp; Metrics</TD></TR>
    </TABLE>
>,fillcolor="#FAD7A0"];
N39 [label=<
    <TABLE BORDER="0" CELLBORDER="1" CELLSPACING="0" CELLPADDING="4" BGCOLOR="#FAD7A0">
        <TR><TD WIDTH="20" ALIGN="CENTER" BGCOLOR="#FAD7A0" BORDER="0" COLOR="#A5B39E">☐</TD><TD WIDTH="100" ALIGN="LEFT" BGCOLOR="#FAD7A0" BORDER="0" COLOR="#A5B39E">Design &amp; rational</TD></TR>
        <TR><TD WIDTH="20" ALIGN="CENTER" BGCOLOR="#FAD7A0" BORDER="0" COLOR="#A5B39E">☐</TD><TD WIDTH="100" ALIGN="LEFT" BGCOLOR="#FAD7A0" BORDER="0" COLOR="#A5B39E">Sim. Logs</TD></TR>
    </TABLE>
>,fillcolor="#FAD7A0"];
N41 [label=<
    <TABLE BORDER="0" CELLBORDER="1" CELLSPACING="0" CELLPADDING="4" BGCOLOR="#FAD7A0">
        <TR><TD WIDTH="20" ALIGN="CENTER" BGCOLOR="#FAD7A0" BORDER="0" COLOR="#A5B39E">☐</TD><TD WIDTH="100" ALIGN="LEFT" BGCOLOR="#FAD7A0" BORDER="0" COLOR="#A5B39E">Environ. Assumptions</TD></TR>
                <TR><TD WIDTH="20" ALIGN="CENTER" BGCOLOR="#FAD7A0" BORDER="0" COLOR="#A5B39E">☐</TD><TD WIDTH="100" ALIGN="LEFT" BGCOLOR="#FAD7A0" BORDER="0" COLOR="#A5B39E">Domain Gap Analysis</TD></TR>
    </TABLE>
>,fillcolor="#FAD7A0"];

N45 [label=<
    <TABLE BORDER="0" CELLBORDER="1" CELLSPACING="0" CELLPADDING="4" BGCOLOR="#FAD7A0">
        <TR><TD WIDTH="20" ALIGN="CENTER" BGCOLOR="#FAD7A0" BORDER="0" COLOR="#A5B39E">☐</TD><TD WIDTH="100" ALIGN="LEFT" BGCOLOR="#FAD7A0" BORDER="0" COLOR="#A5B39E">Scen. Coverage Matrix</TD></TR>
        <TR><TD WIDTH="20" ALIGN="CENTER" BGCOLOR="#FAD7A0" BORDER="0" COLOR="#A5B39E">☐</TD><TD WIDTH="100" ALIGN="LEFT" BGCOLOR="#FAD7A0" BORDER="0" COLOR="#A5B39E">Sim. Training logs</TD></TR>
    </TABLE>
>,fillcolor="#FAD7A0"];
N50 [label=<
    <TABLE BORDER="0" CELLBORDER="1" CELLSPACING="0" CELLPADDING="4" BGCOLOR="#FAD7A0">
        <TR><TD WIDTH="20" ALIGN="CENTER" BGCOLOR="#FAD7A0" BORDER="0" COLOR="#A5B39E">☐</TD><TD WIDTH="100" ALIGN="LEFT" BGCOLOR="#FAD7A0" BORDER="0" COLOR="#A5B39E">Training logs &amp; metrics</TD></TR>
        <TR><TD WIDTH="20" ALIGN="CENTER" BGCOLOR="#FAD7A0" BORDER="0" COLOR="#A5B39E">☐</TD><TD WIDTH="100" ALIGN="LEFT" BGCOLOR="#FAD7A0" BORDER="0" COLOR="#A5B39E">Test results</TD></TR>
    </TABLE>
>,fillcolor="#FAD7A0"];


    // Links
    N1->N20
    {rank=same;N1;N20}
    N20-> {N2,N19,N27}
    N19->N12,N25
    N2 -> N7  
    N2 -> N38
    N3 -> N8 
    N3 -> N44
    N8 -> N9
     N4 -> N6  
    N3 -> N40
    N8 -> N14 
    N9 -> N15 
    N6 -> N16 
    N6 -> N13 
    N11 -> N18 
    N13 -> N17
    N7 -> N3  
    N7 -> N4  
    N12 -> {N22, N11, N26}
    N22 -> N24
    N26->N23
    N27->N28, N29, N30
    N42->N36
    N25->N42
    N25->N49
    N38->N39
    
    N28->N31
    N28->N46
    N28->N48
    N29->N32
    N30->N33
    N31, N32, N46->N34
    N33->N35
    N36->N37
    N40->N41
    N42->N37
     N44->N45
     N48->N35
     N49->N50
 


}




==> figures/tables/dimensions.tex <==


\begin{table*}[t]  % Use table* to span both columns
    \centering
    \setlength{\tabcolsep}{-3pt}
    \caption{Dimensions of Trustworthy RL \& Example \texttt{ASKs}}
    \renewcommand{\arraystretch}{1.6}  % Adjust row height for better spacing
    \setlength{\tabcolsep}{8pt}        % Reduce column padding slightly
    \footnotesize
    \begin{tabular}{|m{0.12\textwidth}||>{\raggedright\arraybackslash}m{0.48\textwidth}|>{\raggedright\arraybackslash}m{0.3\textwidth}|}
        \hline
        \rowcolor{BlueGray} % Blue-gray background for header
        \multicolumn{1}{|c||}{\textbf{\textcolor{black}{Dimension}}} & \textbf{\textcolor{black}{Description}} & \textbf{\textcolor{black}{Example ASK}} \\
        \hline
        \hline
        \centering \parbox{0.12\textwidth}{ \centering \textbf{Robustness} \vspace{0.1em} \\ \includegraphics[width=0.5cm]{figures/icons/robustness.png}} & 
        Focuses on the system's ability to withstand uncertainties, defend against adversarial attacks, and handle discrepancies between the training and deployment environments without a significant drop in performance. & 
        Have potential adversarial scenarios been considered, including perturbations to observations, actions, or rewards? \\
        \hline
        \centering \parbox{0.12\textwidth}{ \centering \textbf{Generalizability} \vspace{0.1em} \\ \includegraphics[width=0.5cm]{figures/icons/generalizability.png}} & 
        Ensures that trained models maintain high performance across a diverse range of previously unseen environments, demonstrating adaptability to both in-domain variations and out-of-domain scenarios. & 
        Does the RL system include mechanisms to detect when the agent encounters out-of-domain states or adversarial scenarios? \\
        \hline
        \centering \parbox{0.12\textwidth}{ \centering \textbf{Safety} \vspace{0.1em} \\ \includegraphics[width=0.5cm]{figures/icons/safety.png}} & 
        Seeks to prevent the execution of actions that could result in catastrophic outcomes by designing policies that rigorously adhere to safety constraints throughout both the training and deployment phases. & 
        Have safety constraints been clearly defined and enforced to prevent the RL agent from entering high-risk states or taking unsafe actions at runtime? \\
        \hline
        \centering \parbox{0.10\textwidth}{\centering \textbf{Transparency} \vspace{0.1em} \\ \includegraphics[width=0.5cm]{figures/icons/transparency.png}} & 
        Encourages decision-making processes, policy behaviors, and system responses that are clear, interpretable, and easily auditable, allowing human overseers to understand and evaluate the system’s actions effectively. & 
        Are rewards, actions, and states exposed to the human overseer during runtime to enhance the interpretability of the agent’s decisions? \\
        \hline
    \end{tabular}
    \vspace{-12pt} \\ 
    \label{tab:dimensions}
\end{table*}


==> figures/tables/full-use-case.tex <==
\begin{table*}[h]
\centering
\begin{tabular}{p{5.5cm}|p{5.5cm}|p{5.5cm}}
\rowcolor{BlueGray} \multicolumn{3}{c}{\textbf{Goal 1: Real-World Readiness \& Adaptability}} \\
\multicolumn{3}{c}{\textbf{\texttt{Subgoal 1.1 Scenario Diversity \& Coverage}}} \\ \midrule

\textbf{\texttt{\uline{ASK 1:}} Have diverse scenarios, including standard operations, irregularities like sensor errors, and edge cases (such as abrupt environmental shifts), been comprehensively identified?} & \textbf{\texttt{\uline{ASK 2:}} Have potential adversarial scenarios been considered, including perturbations to observations, actions, or rewards?} & \textbf{\texttt{\uline{ASK 3:}} In multi-agent settings, have failures or suboptimal behaviors of other agents been considered to ensure individual RL-agents are able to adapt appropriately?} \\ 

\ding{51} \texttt{Yes} \ding{111} \texttt{No} \ding{111} \texttt{N/A} \ding{111} \texttt{?} & \ding{51} \texttt{Yes} \ding{111} \texttt{No} \ding{111} \texttt{N/A} \ding{111} \texttt{?} & \ding{51} \texttt{Yes} \ding{111} \texttt{No} \ding{111} \texttt{N/A} \ding{111} \texttt{?} \\ 

{\small \textbf{Explanation:}} \raggedright \newline  -- \textit{Normal Operations}: Standard path following with dynamic obstacle avoidance \newline  -- \textit{Abnormal Scenarios}: Sudden obstacles, sensor failures, communication delays \newline  -- \textit{Edge Cases}: High-density environments, multiple agent failures, extreme conditions & {\small \textbf{Explanation:}} \newline -- \textit{Anomaly Detection:} Continuous monitoring of state variables (e.g., agent velocities, distances to obstacles) and triggering alerts when thresholds are exceeded. & {\small \textbf{Explanation:}} \newline -- \textit{Detecting Failure:} Heartbeat signals indicate potential failure if absent. \newline -- \textit{Adapt to Failure:} Train agents for resilience and adaptability in unpredictable scenarios. \\ \hline

\multicolumn{3}{c}{\textbf{\texttt{Subgoal 1.2 Design-Environment Alignment}}} \\ \midrule

\multicolumn{3}{p{16.5cm}}{\centering \textbf{\texttt{\uline{ASK 1:}} Does the proposed RL agent align with the environment’s characteristics, such as observability, \newline continuity, and state representation?}} \\ 

\multicolumn{3}{p{16.5cm}}{\centering \ding{51} \texttt{Yes} \ding{111} \texttt{No} \ding{111} \texttt{N/A} \ding{111} \texttt{?}} \\ 

\multicolumn{3}{p{16.5cm}}{{\small \textbf{Explanation:}} \newline -- \textit{Observability:} (a) Partially Observable Markov Decision Processes (POMDPs)  (b) Implement LSTM (for noisy state inputs) \newline -- \textit{Continuous States and Actions:} (a) DDPG} \\ \hline

\multicolumn{3}{c}{\textbf{\texttt{Subgoal 1.3 Resilience \& Adaptation in Real-World Deployment}}} \\ \midrule

\textbf{\texttt{\uline{ASK 5:}} Does the RL system include mechanisms, such as anomaly detection or uncertainty estimation, to detect when the agent encounters out-of-domain states or adversarial scenarios?} & \textbf{\texttt{\uline{ASK 6:}} Is there a pre-defined strategy for handling unexpected scenarios, such as switching to a defined safe mode, halting or deferring to a human overseer?} & \textbf{\texttt{\uline{ASK 7:}} Have the accuracy and reliability of transferring policies from sim-to-real world settings been validated across all critical aspects, including sensor fidelity, environmental dynamics, and latency?} \\ 

\ding{51} \texttt{Yes} \ding{111} \texttt{No} \ding{111} \texttt{N/A} \ding{111} \texttt{?} & \ding{51} \texttt{Yes} \ding{111} \texttt{No} \ding{111} \texttt{N/A} \ding{111} \texttt{?} & \ding{51} \texttt{Yes} \ding{111} \texttt{No} \ding{111} \texttt{N/A} \ding{111} \texttt{?} \\ 

{\small \textbf{Explanation:}} \newline -- \textit{Detection of Adversarial Scenarios:} \newline Mahalanobix Distance-Based OOD Detection: Calculate the Mahalanobis distance of incoming observations from the training distribution to identify OOD scenarios. \newline -- \textit{Anomaly Detection:} Continuous monitoring of state variables (e.g., agent velocities, distances to obstacles) and trigger alerts when values exceed predefined thresholds. & {\small \textbf{Explanation:}} \newline -- \textit{Emergency Stop Mechanism:} \newline $\bullet$ Hard Constraints: Trigger an emergency stop or safe mode when critical safety thresholds (e.g., minimum separation distances) are violated. \newline $\bullet$ Abort Hover followed by Land/Human Control Fail Modes. \newline -- \textit{Fallback Policies:} \newline $\bullet$ A* with real-time obstacle avoidance \newline $\bullet$ Velocity Obstacles & {\small \textbf{Explanation:}} \newline -- \textit{Multi-Tier Training:} \newline 1. Start in low fidelity training (Pygame) \newline 2. Fine-tune on High Fidelity Simulation (Gazebo) \newline 3. Online Training (Real World). Record states, actions, and rewards presented during real-world execution and retrain. \newline -- \textit{Sim-to-Real Transfer Techniques:} \newline Domain Adaptation: Use techniques like domain randomization and transfer learning to reduce the sim-to-real gap. \\ \hline
\end{tabular}
\end{table*}

\begin{table*}[h]
\centering
\begin{tabular}{p{5.5cm}|p{5.5cm}|p{5.5cm}}
\rowcolor{BlueGray} \multicolumn{3}{c}{\textbf{Goal 2: Risk Management}} \\
\multicolumn{3}{c}{\textbf{\texttt{Subgoal 2.1 Risk-Aware Training}}} \\ \midrule

\textbf{\texttt{\uline{ASK 11:}} Do the training and evaluation metrics explicitly include measures across robustness, safety, and generalizability?} & \textbf{\texttt{\uline{ASK 12:}} Are safety constraints explicitly incorporated into the training process to effectively minimize risky behaviors?} & \textbf{\texttt{\uline{ASK 13:}} Does the reward function explicitly prioritize safety, incentivizing stable behavior and penalizing high-risk actions?} \\ 

\ding{51} \texttt{Yes} \ding{111} \texttt{No} \ding{111} \texttt{N/A} \ding{111} \texttt{?} & \ding{51} \texttt{Yes} \ding{111} \texttt{No} \ding{111} \texttt{N/A} \ding{111} \texttt{?} & \ding{51} \texttt{Yes} \ding{111} \texttt{No} \ding{111} \texttt{N/A} \ding{111} \texttt{?} \\ 

{\small \textbf{Explanation:}} \raggedright \newline -- \textit{Training:} \newline 1) States: Do not allow states that violate a minimum distance threshold. Penalize any actions where agents attempt to transition into these ‘not allowed’ states. \newline 2) Constrained Policy Optimization \newline -- \textit{Metrics:} \newline 1) Collision Rate \newline 2) Actions that would result in Minimum Separation Distance violations & {\small \textbf{Explanation:}} \newline -- \textit{Penalize Agent for the following:} \newline 1) Collisions \newline 2) Penalties for violating minimum separation distances, with the penalty magnitude increasing as the violation severity increases & {\small \textbf{Explanation:}} \newline See ASK 12 \\ \hline


\multicolumn{1}{p{\textwidth}}{\textbf{\texttt{\uline{Subgoal 2.2 Proactive Risk Aversion}}}} \\
\multicolumn{1}{p{\textwidth}}{\centering \textbf{\texttt{\uline{ASK 1:}} Placeholder question text for ASK 1.} \newline \ding{111} \texttt{Yes} \ding{111} \texttt{No} \ding{111} \texttt{N/A} \ding{111} \texttt{?}} \\ \midrule

\multicolumn{1}{p{\textwidth}}{\textbf{\texttt{\uline{Subgoal 2.3 Real-Time Risk Detection}}}} \\
\multicolumn{1}{p{\textwidth}}{\centering \textbf{\texttt{\uline{ASK 1:}} Placeholder question text for ASK 1.} \newline \ding{111} \texttt{Yes} \ding{111} \texttt{No} \ding{111} \texttt{N/A} \ding{111} \texttt{?}} \\ \midrule

\multicolumn{1}{p{\textwidth}}{\textbf{\texttt{\uline{Subgoal 2.4 Automatic Overrides and Failsafes}}}} \\
\multicolumn{1}{p{\textwidth}}{\centering \textbf{\texttt{\uline{ASK 1:}} Placeholder question text for ASK 1.} \newline \ding{111} \texttt{Yes} \ding{111} \texttt{No} \ding{111} \texttt{N/A} \ding{111} \texttt{?}} \\ \hline

\end{tabular}
\caption{Complete use-case responses provided by C1.}
\end{table*}

\rowcolor{BlueGray} \multicolumn{1}{c}{\textbf{Goal 3: Human-Centric Alignment \& Control}} \\
\multicolumn{1}{p{\textwidth}}{\textbf{\texttt{\uline{Subgoal 3.1 Human Intervention}}}} \\
\multicolumn{1}{p{\textwidth}}{\centering \textbf{\texttt{\uline{ASK 1:}} Placeholder question text for ASK 1.} \newline \ding{111} \texttt{Yes} \ding{111} \texttt{No} \ding{111} \texttt{N/A} \ding{111} \texttt{?}} \\ \midrule

\multicolumn{1}{p{\textwidth}}{\textbf{\texttt{\uline{Subgoal 3.2 Human Oversight}}}} \\
\multicolumn{1}{p{\textwidth}}{\centering \textbf{\texttt{\uline{ASK 1:}} Placeholder question text for ASK 1.} \newline \ding{111} \texttt{Yes} \ding{111} \texttt{No} \ding{111} \texttt{N/A} \ding{111} \texttt{?}} \\
\multicolumn{1}{p{\textwidth}}{\centering \textbf{\texttt{\uline{ASK 2:}} Placeholder question text for ASK 2.} \newline \ding{111} \texttt{Yes} \ding{111} \texttt{No} \ding{111} \texttt{N/A} \ding{111} \texttt{?}} \\
\multicolumn{1}{p{\textwidth}}{\centering \textbf{\texttt{\uline{ASK 3:}} Placeholder question text for ASK 3.} \newline \ding{111} \texttt{Yes} \ding{111} \texttt{No} \ding{111} \texttt{N/A} \ding{111} \texttt{?}} \\ \midrule

\multicolumn{1}{p{\textwidth}}{\textbf{\texttt{\uline{Subgoal 3.3 Post-Mortem Analysis}}}} \\
\multicolumn{1}{p{\textwidth}}{\centering \textbf{\texttt{\uline{ASK 1:}} Placeholder question text for ASK 1.} \newline \ding{111} \texttt{Yes} \ding{111} \texttt{No} \ding{111} \texttt{N/A} \ding{111} \texttt{?}} \\ \hline
\end{tabular}
\caption{Complete use-case responses provided by C1.}
\end{table*}


==> figures/tables/goal1-res.tex <==
\begin{table*}[h]
\caption{Goal 1 Responses for Case Study by C1}

\label{tab:goal1-res}
\centering
\footnotesize{ % Experimenting with small font
\begin{tabular}{p{5.5cm}|p{5.5cm}|p{5.5cm}}
\rowcolor{BlueGray} \multicolumn{3}{c}{\textbf{Goal 1: Real-World Readiness \& Adaptability}} \\
\multicolumn{3}{c}{\textbf{\texttt{Subgoal 1.1 Scenario Diversity \& Coverage}}} \\ \midrule

\textbf{\texttt{\uline{ASK 1:}} Have diverse scenarios, including standard operations, irregularities like sensor errors, and edge cases (such as abrupt environmental shifts), been comprehensively identified?} & \textbf{\texttt{\uline{ASK 2:}} Have potential adversarial scenarios been considered, including perturbations to observations, actions, or rewards?} & \textbf{\texttt{\uline{ASK 3:}} In multi-agent settings, have failures or suboptimal behaviors of other agents been considered to ensure individual RL-agents are able to adapt appropriately?} \\ 

\ding{51} \texttt{Yes} \ding{111} \texttt{No} \ding{111} \texttt{N/A} \ding{111} \texttt{?} & \ding{51} \texttt{Yes} \ding{111} \texttt{No} \ding{111} \texttt{N/A} \ding{111} \texttt{?} & \ding{51} \texttt{Yes} \ding{111} \texttt{No} \ding{111} \texttt{N/A} \ding{111} \texttt{?} \\ 

{\small \textbf{Explanation:}} \raggedright \newline  -- \textit{Normal Operations}: Standard path following with dynamic obstacle avoidance \newline  -- \textit{Abnormal Scenarios}: Sudden obstacles, sensor failures, communication delays \newline  -- \textit{Edge Cases}: High-density environments, multiple agent failures, extreme conditions & {\small \textbf{Explanation:}} \newline -- \textit{Anomaly Detection:} Continuous monitoring of state variables (e.g., agent velocities, distances to obstacles) and triggering alerts when thresholds are exceeded. & {\small \textbf{Explanation:}} \newline -- \textit{Detecting Failure:} Heartbeat signals indicate potential failure if absent. \newline -- \textit{Adapt to Failure:} Train agents for resilience and adaptability in unpredictable scenarios. \\ \hline

\multicolumn{3}{c}{\textbf{\texttt{Subgoal 1.2 Design-Environment Alignment}}} \\ \midrule

\multicolumn{3}{p{16.5cm}}{\centering \textbf{\texttt{\uline{ASK 0:}} Does the proposed RL agent align with the environment’s characteristics, such as observability, \newline continuity, and state representation?}} \\ 

\multicolumn{3}{p{16.5cm}}{\centering \ding{51} \texttt{Yes} \ding{111} \texttt{No} \ding{111} \texttt{N/A} \ding{111} \texttt{?}} \\ 

\multicolumn{3}{p{16.5cm}}{{\small \textbf{Explanation:}} \newline -- \textit{Observability:} (a) Partially Observable Markov Decision Processes (POMDPs)  (b) Implement LSTM (for noisy state inputs) \newline -- \textit{Continuous States and Actions:} (a) DDPG} \\ \hline

\multicolumn{3}{c}{\textbf{\texttt{Subgoal 1.3 Resilience \& Adaptation in Real-World Deployment}}} \\ \midrule

\textbf{\texttt{\uline{ASK 5:}} Does the RL system include mechanisms, such as anomaly detection or uncertainty estimation, to detect when the agent encounters out-of-domain states or adversarial scenarios?} & \textbf{\texttt{\uline{ASK 6:}} Is there a pre-defined strategy for handling unexpected scenarios, such as switching to a defined safe mode, halting or deferring to a human overseer?} & \textbf{\texttt{\uline{ASK 7:}} Have the accuracy and reliability of transferring policies from sim-to-real world settings been validated across all critical aspects, including sensor fidelity, environmental dynamics, and latency?} \\ 

\ding{51} \texttt{Yes} \ding{111} \texttt{No} \ding{111} \texttt{N/A} \ding{111} \texttt{?} & \ding{51} \texttt{Yes} \ding{111} \texttt{No} \ding{111} \texttt{N/A} \ding{111} \texttt{?} & \ding{51} \texttt{Yes} \ding{111} \texttt{No} \ding{111} \texttt{N/A} \ding{111} \texttt{?} \\ 

{\small \textbf{Explanation:}} \newline -- \textit{Detection of Adversarial Scenarios:} \newline Mahalanobix Distance-Based OOD Detection: Calculate the Mahalanobis distance of incoming observations from the training distribution to identify OOD scenarios. \newline -- \textit{Anomaly Detection:} Continuous monitoring of state variables (e.g., agent velocities, distances to obstacles) and trigger alerts when values exceed predefined thresholds. & {\small \textbf{Explanation:}} \newline -- \textit{Emergency Stop Mechanism:} \newline $\bullet$ Hard Constraints: Trigger an emergency stop or safe mode when critical safety thresholds (e.g., minimum separation distances) are violated. \newline $\bullet$ Abort Hover followed by Land/Human Control Fail Modes. \newline -- \textit{Fallback Policies:} \newline $\bullet$ A* with real-time obstacle avoidance \newline $\bullet$ Velocity Obstacles & {\small \textbf{Explanation:}} \newline -- \textit{Multi-Tier Training:} \newline 1. Start in low fidelity training (Pygame) \newline 2. Fine-tune on High Fidelity Simulation (Gazebo) \newline 3. Online Training (Real World). Record states, actions, and rewards presented during real-world execution and retrain. \newline -- \textit{Sim-to-Real Transfer Techniques:} \newline Domain Adaptation: Use techniques like domain randomization and transfer learning to reduce the sim-to-real gap. 
\\
\hline
\multicolumn{3}{c}{} \\ % This adds an empty row with no lines
\end{tabular}

\end{table*}


==> figures/tables/goal2-res.tex <==
\begin{table*}[h]
\caption{Goal 2 Responses for Case Study by C1}
\label{tab:goal2-res}
\footnotesize
\centering
\begin{tabular}{p{5.5cm}|p{5.5cm}|p{5.5cm}}
\rowcolor{BlueGray} \multicolumn{3}{c}{\textbf{Goal 2: Risk Management}} \\
\multicolumn{3}{c}{\textbf{\texttt{Subgoal 2.1 Risk-Aware Training}}} \\ \midrule

\textbf{\texttt{\uline{ASK 11:}} Do the training and evaluation metrics explicitly include measures across robustness, safety, and generalizability?} & \textbf{\texttt{\uline{ASK 12:}} Are safety constraints explicitly incorporated into the training process to effectively minimize risky behaviors?} & \textbf{\texttt{\uline{ASK 13:}} Does the reward function explicitly prioritize safety, incentivizing stable behavior and penalizing high-risk actions?} \\ 

\ding{51} \texttt{Yes} \ding{111} \texttt{No} \ding{111} \texttt{N/A} \ding{111} \texttt{?} & \ding{51} \texttt{Yes} \ding{111} \texttt{No} \ding{111} \texttt{N/A} \ding{111} \texttt{?} & \ding{51} \texttt{Yes} \ding{111} \texttt{No} \ding{111} \texttt{N/A} \ding{111} \texttt{?} \\ 

{\small \textbf{Explanation:}} \raggedright \newline -- \textit{Training:} \newline 1) States: Do not allow states that violate a minimum distance threshold. Penalize any actions where agents attempt to transition into these ‘not allowed’ states. \newline 2) Constrained Policy Optimization \newline -- \textit{Metrics:} \newline 1) Collision Rate \newline 2) Actions that would result in Minimum Separation Distance violations & {\small \textbf{Explanation:}} \newline -- \textit{Penalize Agent for the following:} \newline 1) Collisions \newline 2) Penalties for violating minimum separation distances, with the penalty magnitude increasing as the violation severity increases & {\small \textbf{Explanation:}} \newline See ASK 12 \\ \hline

\multicolumn{3}{c}{\textbf{\texttt{Subgoal 2.2 Proactive Risk Aversion}}} \\ \midrule

\multicolumn{3}{p{16.5cm}}{\textbf{\texttt{\uline{ASK 10:}} Have safety constraints been clearly defined and enforced to prevent the RL agent from entering high-risk states or taking unsafe actions at runtime?}} \\ 

\multicolumn{3}{p{16.5cm}}{\ding{51} \texttt{Yes} \ding{111} \texttt{No} \ding{111} \texttt{N/A} \ding{111} \texttt{?}}\\ 

\multicolumn{3}{p{16.5cm}}{{\small \textbf{Explanation:}} \raggedright \newline -- \textit{Minimum Separation Distances:} Define and enforce minimum separation constraints between agents and obstacles. \newline -- \textit{Speed and Acceleration Limits:} Set maximum allowable speeds and acceleration to prevent loss of control. \newline -- \textit{Operational Boundaries:} Define areas where agents should not operate, similar to a geofence.}\\ \hline

\end{tabular}



\begin{tablenotes}
    \small \textit{* To conserve space, only unique responses are included as two of the ASKs had similar explanations as those from Goal 1}
\end{tablenotes}

\end{table*}


==> figures/tables/goal3-res.tex <==
\begin{table*}
\caption{Goal 2 Responses for Case Study by C1}
\label{tab:goal3-res}
\centering
\footnotesize{ % Experimenting with small font
\begin{tabular}{p{5.5cm}|p{5.5cm}|p{5.5cm}}
\rowcolor{BlueGray} \multicolumn{3}{c}
{\textbf{Goal 3: Human-Centric Alignment \& Control}} \\
\multicolumn{3}{c}{\textbf{\texttt{Subgoal 3.1 Human Intervention}}} \\ \midrule

\multicolumn{3}{p{16.5cm}}{\textbf{\texttt{\uline{ASK 18:}} Have human interventions been identified \& supported by affordances?}} \\ 

\multicolumn{3}{p{16.5cm}}{\ding{51} \texttt{Yes} \ding{111} \texttt{No} \ding{111} \texttt{N/A} \ding{111} \texttt{?}}\\ 

\multicolumn{3}{p{16.5cm}}{{\small \textbf{Explanation:}} \raggedright \newline -- \textit{Manual Override Controls:} \newline 1) Human operator can take control at any time. \newline 2) Human operator can opt out any agent out of the RL system and fall back to fail-safe or human control.} \\ \hline

\multicolumn{3}{c}{\textbf{\texttt{Subgoal 3.2 Human Oversight}}} \\ \midrule

\textbf{\texttt{\uline{ASK 15:}} If possible, is the human overseer actively involved in shaping the training process to enhance transparency \& promote alignment with specific safety \& operation goals?} & \textbf{\texttt{\uline{ASK 16:}} Are critical factors or states that significantly impact behavior and safety highlighted for the human overseer?} & \textbf{\texttt{\uline{ASK 17:}} Are rewards, actions, and states exposed to the human overseer during runtime to enhance the interpretability of the agent’s decisions?} \\ 

\ding{111} \texttt{YES} \ding{55} \texttt{No} \ding{111} \texttt{N/A} \ding{111} \texttt{?} & \ding{51} \texttt{Yes} \ding{111} \texttt{No} \ding{111} \texttt{N/A} \ding{111} \texttt{?} & \ding{51} \texttt{Yes} \ding{111} \texttt{No} \ding{111} \texttt{N/A} \ding{111} \texttt{?} \\ 

{\small \textbf{Explanation:}} \newline Other than the initial design of states, actions, and rewards, there is no additional human input that shapes the training process. & {\small \textbf{Explanation:}} \newline -- \textit{Display Proposed Paths:} Display proposed paths for each agent onto the GUI. \newline -- \textit{Minimum Separation Distances:} Display the minimum separation distance for each drone at each epoch onto the GUI. \newline -- \textit{Events/RL Errors:} Display events or RL errors onto the GUI, such as when an RL agent is stuck on a local minima and needs to transition to a fail-safe. & {\small \textbf{Explanation:}} \newline Yes, both during runtime via GUI and logged persistently. \\ \hline


\multicolumn{3}{c}{\textbf{\texttt{Subgoal 3.3 Post-Mortem Analysis}}} \\ \midrule

\multicolumn{3}{p{16.5cm}}{\textbf{\texttt{\uline{ASK 14:}} Are clear and detailed logs, metrics, and indicators available to trace decision-making and facilitate analysis of issues post-mortem?}} \\ 

\multicolumn{3}{p{16.5cm}}{\ding{51} \texttt{Yes} \ding{111} \texttt{No} \ding{111} \texttt{N/A} \ding{111} \texttt{?}}\\ 

\multicolumn{3}{p{16.5cm}}{{\small \textbf{Explanation:}} \raggedright \newline -- \textit{State, Action, Rewards Logging:} Record states, actions, rewards, and their corresponding state transitions for each agent, all timestamped. \newline -- \textit{Drone Telemetry Data:} Record drone telemetry data, including position, velocity, and orientation. \newline -- \textit{Event Categorization:} Categorize events as normal operations, constraint violations, or system alerts. \newline -- \textit{Performance and Safety Metrics:} Log metrics like path efficiency, time to destination, and minimum separation distance violations (or actions that would have led to such violations, as fail-safes will prevent any unsafe action). \newline -- \textit{Replay System:} Implement a replay system to view drone state transitions and their actions.} \\ \hline

\end{tabular}


\end{table*}


==> figures/tables/use-case-descr.tex <==
% Table 1: Use Case Descriptions
\begin{table}[!ht]
\centering
\renewcommand{\arraystretch}{1.5}
\setlength{\tabcolsep}{4pt}  % Adjust column padding to fit in one column
\footnotesize
\begin{tabular}{p{1.5cm} p{5cm}}
\toprule
\textbf{Use-Case 1}  &  Multi-agent Path Planning with Dynamic Obstacles \& Minimum Separation Distance Constraints \\
\vspace{1pt}\textbf{Use-Case 2}  & \vspace{1pt} Multi-agent sUAS Path Planning with Battery Efficiency \& Route Optimization \\
\vspace{1pt}\textbf{Use-Case 3} & \vspace{1pt}[Description Needed] \\
\bottomrule
\end{tabular}
\caption{Use Case Descriptions}
\label{tab:use-case-descriptions}
\end{table}

==> figures/tables/use-case-descriptions.tex <==
% \begin{table}[b]
% \caption{\framework was applied to three use-cases in varying degrees of design and implementation.}
% \label{tab:use-cases}
% \centering
% \footnotesize

% \setlength{\tabcolsep}{6pt} % Adjust column spacing for better appearance
% \renewcommand{\arraystretch}{1.3} % Adjust row height for readability

% \begin{tabular}{p{0.2cm} p{4cm} p{3.5cm}}
%     \hline
%     \textbf{ID} & \textbf{Use-Case} & \textbf{Status} \\
%     \hline
%     C1 & Collision avoidance between sUAS whereby Minimum-Separation Distance is computed based upon sensor data providing airspace awareness. 
%        & Preliminary system originally deployed using heuristic approach, with current design representing an RL-based replacement. \\ 
%     \hline
%     C2 & sUAS navigation through a congested area for route optimization and battery efficiency 
%        & Represents a generalization of a previously designed and prototyped system. \\ 
%     \hline
%     E1 & Command and Control of small autonomous ground vehicles& Prototyped \\ 
%     \hline
%     \multicolumn{3}{l}{\footnotesize *C=co-author; E=external expert} \\ % Adjusted alignment and font size
% \end{tabular}
% \vspace{-1em}
% \end{table}

==> figures/ui.tex <==
\begin{figure}[t]
    \centering
    % First subfigure
    
   
    \begin{subfigure}[b]{\columnwidth}  % Adjust the width as needed
        \centering
                
        \includegraphics[width=\linewidth]{figures/images/example-ask.png}
        \caption{View of an \texttt{ASK} node in the tool.}
        \label{fig:ask-node}
    \end{subfigure}
    \vspace{1em} % Add vertical space between the subfigures

    % Second subfigure
    \begin{subfigure}[b]{\columnwidth}  % Adjust the width as needed
        \centering
                
        \includegraphics[width=\textwidth]{figures/images/example-evidence.png}
        \caption{View of an evidence node in the tool.}
        \label{fig:evidence-node}
    \end{subfigure}
    \caption{Visualization of \texttt{ASK} \& evidence nodes in the tool.}
    \label{fig:ui}
    \vspace{-12pt}
\end{figure}

==> notes.tex <==
digraph SafetyArguments {
    node [shape=rect, style=filled, fontname="Helvetica", fontsize=16, fillcolor="#D3D3D3"];  // Default pale gray fill
    edge [fontname="Helvetica", fontsize=14];  // Common edge style
    ranksep=.6
    nodesep=.1
    
    

    // Root node
    T1[label=<
    <TABLE BORDER="0" CELLBORDER="1" CELLSPACING="0" CELLPADDING="4" BGCOLOR="white">
    <TR><TD ALIGN="CENTER" BGCOLOR="#D3D3D3" BORDER="1" COLOR="#A9A9A9"><b>GOAL 1: <BR/>Training Scenarios</b></TD></TR>
    <TR><TD ALIGN="CENTER" BGCOLOR="#D3D3D3" BORDER="1" COLOR="#A9A9A9">Training scenarios <BR/> are close to the real world</TD></TR>
    </TABLE>
    >, fillcolor="white", color="white"]; 
    
    S1[margin=0, width=3.6, height=1.4, shape=polygon, fixedsize=true, label="<Strategy>\nArgue that risks associated\n with mismatched training \nscenarios have been \nidentified and addressed.", skew=0.1];

    T1 ->S1 [dir="back"]
    
    // Sub-claims for Claim 1
    T2[label=<
    <TABLE BORDER="0" CELLBORDER="1" CELLSPACING="0" CELLPADDING="4" BGCOLOR="white">
    <TR><TD ALIGN="CENTER" BGCOLOR="#D3D3D3" BORDER="1" COLOR="#A9A9A9"><b>Subgoal 1.1: <BR/>Scenario Variety</b></TD></TR>
    <TR><TD ALIGN="CENTER" BGCOLOR="#D3D3D3" BORDER="1" COLOR="#A9A9A9">Training covers <BR/>all identified scenarios <BR/>following indepth analysis</TD></TR>
    </TABLE>
    >, fillcolor="white", color="white"];


    T3[label=<
    <TABLE BORDER="0" CELLBORDER="1" CELLSPACING="0" CELLPADDING="4" BGCOLOR="white">
    <TR><TD ALIGN="CENTER" BGCOLOR="#D3D3D3" BORDER="1" COLOR="#A9A9A9"><b>Subgoal 1.2: <BR/>Novel Scenarios</b></TD></TR>
    <TR><TD ALIGN="CENTER" BGCOLOR="#D3D3D3" BORDER="1" COLOR="#A9A9A9">The system will detect &amp; <BR/>handle novel scenarios <BR/>at runtime.</TD></TR>
    </TABLE>
    >, fillcolor="white", color="white"];


    T4[label=<
    <TABLE BORDER="0" CELLBORDER="1" CELLSPACING="0" CELLPADDING="4" BGCOLOR="white">
    <TR><TD ALIGN="CENTER" BGCOLOR="#D3D3D3" BORDER="1" COLOR="#A9A9A9"><b>Subgoal 1.3: <BR/>Deviant Behavior</b></TD></TR>
    <TR><TD ALIGN="CENTER" BGCOLOR="#D3D3D3" BORDER="1" COLOR="#A9A9A9">The system detects &amp;<BR/>handles deviant behavior</TD></TR>
    </TABLE>
    >, fillcolor="white", color="white"];

    S1 -> {T2,T3,T4} [dir="back"]

    // Claim 2: Unsafe Actions
    T5[label=<
    <TABLE BORDER="0" CELLBORDER="1" CELLSPACING="0" CELLPADDING="4" BGCOLOR="white">
    <TR><TD ALIGN="CENTER" BGCOLOR="#D3D3D3" BORDER="1" COLOR="#A9A9A9"><b>Claim 2: Unsafe Actions</b></TD></TR>
    <TR><TD ALIGN="CENTER" BGCOLOR="#D3D3D3" BORDER="1" COLOR="#A9A9A9">Are there safety constraints<BR/>to prevent dangerous actions?</TD></TR>
    </TABLE>
    >, fillcolor="white", color="white"]; 

    // Sub-claims for Claim 2
    T6[label=<
    <TABLE BORDER="0" CELLBORDER="1" CELLSPACING="0" CELLPADDING="4" BGCOLOR="white">
    <TR><TD ALIGN="CENTER" BGCOLOR="#D3D3D3" BORDER="1" COLOR="#A9A9A9"><b>Claim 2.1: Exploration Safety</b></TD></TR>
    <TR><TD ALIGN="CENTER" BGCOLOR="#D3D3D3" BORDER="1" COLOR="#A9A9A9">What limits exist on unsafe<BR/>actions during exploration?</TD></TR>
    </TABLE>
    >, fillcolor="white", color="white"];

    T5 -> T6 [dir="back"]

 
    T7[label=<
    <TABLE BORDER="0" CELLBORDER="1" CELLSPACING="0" CELLPADDING="4" BGCOLOR="white">
    <TR><TD ALIGN="CENTER" BGCOLOR="#D3D3D3" BORDER="1" COLOR="#A9A9A9"><b>Claim 2.2: Reward &amp; Safety</b></TD></TR>
    <TR><TD ALIGN="CENTER" BGCOLOR="#D3D3D3" BORDER="1" COLOR="#A9A9A9">Is safety balanced in the<BR/>reward function?</TD></TR>
    </TABLE>
    >, fillcolor="white", color="white"];
   

    T5 -> T7 [dir="back"]

    T8[label=<
    <TABLE BORDER="0" CELLBORDER="1" CELLSPACING="0" CELLPADDING="4" BGCOLOR="white">
    <TR><TD ALIGN="CENTER" BGCOLOR="#D3D3D3" BORDER="1" COLOR="#A9A9A9"><b>Claim 2.3: Guardrails</b></TD></TR>
    <TR><TD ALIGN="CENTER" BGCOLOR="#D3D3D3" BORDER="1" COLOR="#A9A9A9">What guardrails exist to limit<BR/>unsafe actions in operation?</TD></TR>
    </TABLE>
    >, fillcolor="white", color="white"];

    T5 -> T8 [dir="back"]

    // Claim 3: Post-deployment Safety
    T9[label=<
    <TABLE BORDER="0" CELLBORDER="1" CELLSPACING="0" CELLPADDING="4" BGCOLOR="white">
    <TR><TD ALIGN="CENTER" BGCOLOR="#D3D3D3" BORDER="1" COLOR="#A9A9A9"><b>Claim 3: Post-deployment</b></TD></TR>
    <TR><TD ALIGN="CENTER" BGCOLOR="#D3D3D3" BORDER="1" COLOR="#A9A9A9">How is post-deployment<BR/>learning monitored?</TD></TR>
    </TABLE>
    >, fillcolor="white", color="white"]; 

    // Sub-claims for Claim 3
    T10[label=<
    <TABLE BORDER="0" CELLBORDER="1" CELLSPACING="0" CELLPADDING="4" BGCOLOR="white">
    <TR><TD ALIGN="CENTER" BGCOLOR="#D3D3D3" BORDER="1" COLOR="#A9A9A9"><b>Claim 3.1: New Behaviors</b></TD></TR>
    <TR><TD ALIGN="CENTER" BGCOLOR="#D3D3D3" BORDER="1" COLOR="#A9A9A9">How are new behaviors<BR/>tested before deployment?</TD></TR>
    </TABLE>
    >, fillcolor="white", color="white"];

    T9 -> T10 [dir="back"]

    T11[label=<
    <TABLE BORDER="0" CELLBORDER="1" CELLSPACING="0" CELLPADDING="4" BGCOLOR="white">
    <TR><TD ALIGN="CENTER" BGCOLOR="#D3D3D3" BORDER="1" COLOR="#A9A9A9"><b>Claim 3.2: Unsafe Learning</b></TD></TR>
    <TR><TD ALIGN="CENTER" BGCOLOR="#D3D3D3" BORDER="1" COLOR="#A9A9A9">How is unsafe post-<BR/>deployment learning prevented?</TD></TR>
    </TABLE>
    >, fillcolor="white", color="white"];

    T9 -> T11 [dir="back"]

    // Claim 4: Formal Guarantees & Redundancy
    T12[label=<
    <TABLE BORDER="0" CELLBORDER="1" CELLSPACING="0" CELLPADDING="4" BGCOLOR="white">
    <TR><TD ALIGN="CENTER" BGCOLOR="#D3D3D3" BORDER="1" COLOR="#A9A9A9"><b>Claim 4: Formal Methods</b></TD></TR>
    <TR><TD ALIGN="CENTER" BGCOLOR="#D3D3D3" BORDER="1" COLOR="#A9A9A9">What formal methods ensure<BR/>the safety of RL decisions?</TD></TR>
    </TABLE>
    >, fillcolor="white", color="white"]; 

    // Sub-claims for Claim 4
    T13[label=<
    <TABLE BORDER="0" CELLBORDER="1" CELLSPACING="0" CELLPADDING="4" BGCOLOR="white">
    <TR><TD ALIGN="CENTER" BGCOLOR="#D3D3D3" BORDER="1" COLOR="#A9A9A9"><b>Claim 4.1: Redundancy</b></TD></TR>
    <TR><TD ALIGN="CENTER" BGCOLOR="#D3D3D3" BORDER="1" COLOR="#A9A9A9">What fallback mechanisms<BR/>exist if formal guarantees fail?</TD></TR>
    </TABLE>
    >, fillcolor="white", color="white"];

    T12 -> T13 [dir="back"]

    // Add more claims here if necessary following this pattern

}

